Towards Auditable Distributed Systems

The emerging trend towards distributed (cloud) systems (DS) has widely arrived whether in the automotive, public or the financial sector, but the execution of services of heterogeneous service providers is exposed to several risks. Beside hardware/software faults or cyber attacks that can influence the correctness of the system, fraud is also an issue. In such case it is not only important to verify the correctness of the system, but also have evidence which component and participant behaves faulty. This makes it possible, e.g. to claim for compensation after systems execution but also to assure information for verification can be trusted. The main goal of our research is to assure the monitoring of DS based on auditable information. We follow a decentralized monitoring strategy and envision a distributed monitoring approach of system properties based on distributedlogic programs that consider auditability. The expected contribution of this work is to establish with the application of our framework the mutual trust of distributed parties, as well as trust of clients in the systems execution. We showcase our ideas on a DS for booking services with unmanned air vehicles.

==> TODO.tex <==
- Check: mehr Unterbrechungen

% HEADER 

- Titel konkreter
- Grant/FKZ: 20X1736M
- Aufzaehlen was monitor macht


==> content/limitations.tex <==
\subsection{Limitations and Challenges}


==> feedback.tex <==
=== Reviewer 1 ===
This paper addresses the objective of auditing huge processed events in distributed systems at runtime, in a generic way.
According to the authors, Runtime auditing of distributed systems is motivated by the need to react immediately in case of misbehavior. One of the requirements of such an auditing process is scalability.

The proposed solution is built on 4 steps. The first one consists to express the monitorable properties in a specification language. The second consists in choosing a verification mechanism. The third is to generate a suitable monitor according to the rules specified in step 1 and finally, the last step consists in storing all the events in a common legger for further verification.

The originality of this solution is in its ability to adapt to different situations but the paper do not give any insights into the requirements a system should have to be a candidate to such a system.

Moreover for step 2: which solution is better for which situation? is it an objective to fix that during the thesis?

The paper is interesting but the scope of application of such a solution should be more precised.


Some points to enhance the paper

- the paper outline is missing: is this necessary?

Score: weak accept

=== Reviewer 2 ===
# Strengths:
- The auditability topic is very interesting
- The paper proposes advancing auditability by moving from a posteriori auditability to online auditability.
- The authors have already implemented a prototype with some components already in place (e.g., Datalog and Trillian).

# Weaknesses:
- The title is too generic for what the paper actually proposes.

- The fault model could be more elaborated. For instance, is it reasonable trusting the cloud to run unreplicated monitors if clouds are untrusted to run unreplicated distributed programs? good point

- It is unclear why other solutions cannot be adapted to audit systems in runtime.

- The system seems to work only on auditing web services, which is a system model restriction that prevents auditability in many other systems that do not use web servers.

- In practical terms, the costs of runtime auditability may be too high. What are the properties that influence this performance? (e.g., the size of the logs? the complexity of log records?)

- What is the required event ordering (e.g., strict, causal)? Can logical clocks solve the problem with the order of events?

- What is the security impact of providing the services' private keys to Kubernetes?

# Typos:

- Some references (e.g., [18, 24]) do not have where they were published.

# Score: weak accept


=== Reviewer 3 ===
The paper presents an interesting idea to make distributed systems auditable at runtime by using distributed monitors.
The idea is interesting and the paper is well written  ( also including some research questions).
On the other hand, the work is really preliminary work. The paper is not supported by quantitative data and it is not clear if some experiments using real-world data are performed to prove the validity of the approach compared with existing solutions.

Strenghts
    -The paper addresses an interesting topic
    -The paper is well written

Score: borderline paper

==> sketch.tex <==
- Problem when logging is not correctly of a monitor

- Accessability of a component to connect to monitor

- Consider runtime monitoring as a technique for gaining auditability
